Robust Analysis of Multi-Task Learning Efficiency: New Benchmarks on Light-Weighed Backbones and Effective Measurement of Multi-Task Learning Challenges by Feature Disentanglement

One of the main motivations of MTL is to develop neural networks capable of inferring multiple tasks simultaneously. While countless methods have been proposed in the past decade investigating robust model architectures and efficient training algorithms, there is still lack of understanding of these methods when applied on smaller feature extraction backbones, the generalizability of the commonly used fast approximation technique of replacing parameter-level gradients with feature level gradients, and lack of comprehensive understanding of MTL challenges and how one can efficiently and effectively identify the challenges. In this paper, we focus on the aforementioned efficiency aspects of existing MTL methods. We first carry out large-scale experiments of the methods with smaller backbones and on a the MetaGraspNet dataset as a new test ground. We also compare the existing methods with and without using the fast gradient surrogate and empirically study the generalizability of this technique. Lastly, we propose Feature Disentanglement measure as a novel and efficient identifier of the challenges in MTL, and propose Ranking Similarity score as an evaluation metric for different identifiers to prove the faithfulness of our method.

==> sections/2_related_work/architecture.tex <==
\subsection{Network Design}

We briefly cover the existing research on network architecture design without going into too much details, as this is not the focus of our work. The application of this concept of multi-task learning is also not a recent thing \cite{overfeat, fastrcnn, maskrcnn, eigen2015predicting, liao2016understand, hyperface, uhrig2016pixel, multinet, ubernet, neven2017fast, blitznet, mohamed2021spatio}. More advanced designs include feature fusion methods \cite{crossresidual, yang2016trace, crossstitch, sluice, nddr, crossinfonet}, feature selection (attention mechanism) \cite{mtan, maninis2019attentive, mult}, task information distillation \cite{padnet, trl, zhao2018modulation, pap, mtinet}, knowledge distillation \cite{xu2023multi, ye2023taskexpert, chen2023adamv, jacob2023online}, and neural architecture search \cite{lu2017fully, vandenhende2019branched, guangyuan2022recon, guo2020learning, raychaudhuri2022controllable, sun2020adashare, gao2020mtl, choi2023dynamic, dong2018dpp}.

% \noindent\textbf{Feature Fusion} methods \cite{crossresidual, yang2016trace, crossstitch, sluice, nddr, crossinfonet}, or soft parameter sharing, start from single-task networks or branches designed for individual tasks, and then add feature fusion modules to fuse the representations learned by each branch. This line of research assumes a fixed network topology and focus on developing various inter-branch connections.

% \noindent\textbf{Feature Selection} methods \cite{mtan, maninis2019attentive, mult}, or attention mechanisms, aim to insert ``add-ons'' to neural networks to weigh intermediate features. This is effectively selecting useful features for each down-stream task. The most common form is to design (local) two-branch networks, similar to residual connections \cite{resnet}, where the additional branch is responsible for generating weights to be applied on the features on the identity branch.

% \noindent\textbf{Task Information Distillation} methods \cite{padnet, trl, zhao2018modulation, pap, mtinet} are still architecture designs at the core, but utilizes the idea that task-specific features could be useful for each other if given as input to the decoder. So these works make models to predict for each task sequentially, rather than in parallel, and the output of an earlier task would become the input of a later one.

% \noindent\textbf{Knowledge Distillation} methods \cite{xu2023multi, ye2023taskexpert, chen2023adamv, jacob2023online} propose to distill the information from teacher networks into a student multi-task network, where the teacher networks could be just another multi-task network \cite{xu2023multi}, a mixture of expert networks \cite{ye2023taskexpert, chen2023adamv}, or single-task networks \cite{jacob2023online}.

% \noindent\textbf{Neural Architecture Search}.
% In contrast, another line of research \cite{lu2017fully, vandenhende2019branched, guangyuan2022recon, guo2020learning, raychaudhuri2022controllable, sun2020adashare, gao2020mtl, choi2023dynamic, dong2018dpp} focuses on architecture design and algorithmic-ally answers the question of ``what to share''. The result of architecture search is commonly known as ``hard parameter sharing'' schemes in the literature. Affinity-based approaches \cite{lu2017fully, vandenhende2019branched, guangyuan2022recon} first measure task affinity scores and design the network so that highly correlated tasks are processed in the same branch. Gradient-based approaches \cite{guo2020learning, raychaudhuri2022controllable, sun2020adashare, gao2020mtl} jointly fine-tuning the network parameters and a parameterized distribution over a pre-defined search space by minimizing the same loss functions.


==> sections/2_related_work/meta_learning.tex <==
\subsection{Meta Learning}

\cite{ye2021multi}

